How Feasible is Augmenting Fake Nodes with Learnable Features as a Counter-strategy against Link Stealing Attacks?

Graph Neural Networks (GNNs) are widely used and deployed for graph-based prediction tasks. However, as good as GNNs are for learning graph data, they also come with the risk of privacy leakage. For instance, an attacker can run carefully crafted queries on the GNNs and, from the responses, can infer the existence of an edge between a pair of nodes. This attack, dubbed as a "link-stealing" attack, can jeopardize the user's privacy by leaking potentially sensitive information. To protect against this attack, we propose an approach called "$(N)$ode $(A)$ugmentation for $(R)$estricting $(G)$raphs from $(I)$nsinuating their $(S)$tructure" ($NARGIS$) and study its feasibility. $NARGIS$ is focused on reshaping the graph embedding space so that the posterior from the GNN model will still provide utility for the prediction task but will introduce ambiguity for the link-stealing attackers. To this end, $NARGIS$ applies spectral clustering on the given graph to facilitate it being augmented with new nodes -- that have learned features instead of fixed ones. It utilizes tri-level optimization for learning parameters for the GNN model, surrogate attacker model, and our defense model (i.e. learnable node features). We extensively evaluate $NARGIS$ on three benchmark citation datasets over eight knowledge availability settings for the attackers. We also evaluate the model fidelity and defense performance on influence-based link inference attacks. Through our studies, we have figured out the best feature of $NARGIS$ -- its superior fidelity-privacy performance trade-off in a significant number of cases. We also have discovered in which cases the model needs to be improved, and proposed ways to integrate different schemes to make the model more robust against link stealing attacks.

==> codaspyTex/extra_perturbedGNN.tex <==
\subsection{Perturbed Graph Embedding Learning Module}
After learning the augmented node features, we again reinitialize the target GNN model and learn its parameters again by training on the augmented graph, %in the \module{Perturbed Graph Embedding Module}, 
as shown in \Cref{fig:nargis_overview}. Unlike previous module, the feature of the augmented nodes are not updated in each training step, rather they are fixed. This facilitates the stability of the embedding model. After training, the module returns the node posteriors of the augmented graph. As the attacker is not supposed to know the presence of the defensive measures, hence the augmented nodes' posteriors are not sent as an output of the model. %The model architecture is as same as the \textit{Target GNN Model} stated in \Cref{sec:targetgnn}. %In fact, this is the model whose posteriors are sent to the users, not the \textit{Augmented Target GNN Model}'s one.
The module's operation is described 
 in \Cref{func:perturbgraphembed} in \Cref{app:func}.%, which is as same as the one which we would have run to learn the GNN model without any defense measures. 

%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%

\begin{func}
\caption{learnPerturbedGraphEmbedding$(G_{aug}^{\tau})$}\label[func]{func:perturbgraphembed}
\renewcommand{\arraystretch}{1}
 \fontsize{8}{8}\selectfont
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
\Input{Learned Augmented Graph, $G_{aug}^{\tau} = (V_{aug}, \textbf{X}_{aug}^{\tau}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$;\\}
\Output{Perturbed Node Posteriors from Learned Augmented Graph, $\Phi_{aug} \in [0,1]^{n_{aug} \times c}$ \\}
Learn GNN model
$f(G_{aug}^{\tau}; \theta_f^{\tau}): G_{aug}^{\tau} \rightarrow [0,1]^{n_{aug} \times c}$\; \Comment{$\theta_{f}^{\tau}$ are learnable parameters}
$\Phi_{aug} \gets f(G_{aug}^{\tau}; \theta_f^{\tau})$\;
\Return{$\Phi_{aug}$}
\end{func}




==> codaspyTex/extra_surrogatedataset.tex <==
\subsection{\textbf{Surrogate Dataset Generator Module}}


The aim of \module{Surrogate Dataset Generator Module} (see \Cref{fig:nargis_overview}), is to generate a surrogate dataset for our surrogate attacker model to learn from. 
%\imtiaz{Why pre-processing?}
The dataset consists partially of the edges from the main graph and negative (non-existent) edges sampled from the graph. The goal of this module is to simulate and approximate the attacker's possible training of a surrogate dataset. 
%The module is demonstrated in \Cref{fig:nargis_overview}.
\paragraph{Graph Variational Auto-Encoder}
To simulate the attacker, we need a \textit{ground-truth provider} for learning the \textit{surrogate attacker model} in a supervised manner. For this, we adopt another surrogate model $\psi(.)$ as proxy-ground truth providing dataset for the attacker for edge prediction task. 
In our case, we use a surrogate Graph Variational Auto-Encoder(GVAE) model as an approximation or proxy for the ground-truth provider. For an edge $(u,v) \in E$, $\psi(.)$ or its internal layers can predict whether the edge exists. For GVAE, the encoder's latent representation for the nodes $u, v$ is passed through the inner-product and sigmoid layer to determine the probability of the edge's existence. The set of learnable model parameters of the GVAE is denoted as ${\theta_\psi}$.
    
\Cref{func:getSurrQueryEdgeData} in \Cref{app:func} creates the
%performs the formation of 
surrogate edge query dataset in this module. Formally, the \textit{Surrogate Edge Query Dataset} %\begin{align}\mathcal{D}_Q = \{(u,v, y)| u \in V, v \in V, y = \textbf{A}_{uv}\}\end{align} 
is the set of pairs of nodes as edge endpoints and the binary indicator variable $y$ for the edge. To create the Surrogate Edge Query Dataset, we take all or a portion of the positive edges and negative-sampled non-existing edges from the original graph and pass it through the ground-truth provider $\psi(.)$ to get the label. Formally, 
%
{\small
\begin{align}
 \mathcal{D}_Q = \{(u, v, y)| u \in V, v \in V, y = [\psi(u,v) > \zeta]\}    
\end{align}\label{eq:dq} 
}
%
where $\zeta \in [0,1]$ is a threshold value. 
%COMMENT(FIXED): The term "Ideally" is confusing. The reader does not understand whether you used 0.5 or used a different approach. %MIRCOMMENT: FIXED
We have set $\zeta =0.5$ in our experiments. Empirically, like any other VAE, we used a sampling layer, and we only used minimum-squared losses and no KL divergence while calculating the loss function. The procedure has been described in \Cref{func:getSurrQueryEdgeData} in \Cref{app:func}.

%%%%%%%%%%%%%%%%
\begin{func}

\caption{generateSurrogateEdgeQueryDataset$(G)$}\label[func]{func:getSurrQueryEdgeData}
\renewcommand{\arraystretch}{1}
 \fontsize{8}{8}\selectfont
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Parameter}{Parameter}
\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
\Input{Graph $G = (V, \textbf{X}, \textbf{Y}, \textbf{A}, n, c);$\\}
\Parameter{Set Threshold $\zeta$;\\}
\Output{Surrogate Query Edge Dataset $\mathcal{D}_{Q}$}
$E \gets $ Edges from $G$\;
$E_{train}^{pos} \gets$ positive train split edges from $E$\;
$E_{train}^{neg} \gets$ negative edges sampled from $E$\;
Learn GVAE $\psi(.)$ from $V, E_{train}^{pos} \text{ \& } E_{train}^{neg}$\;
$E_{big} \gets E \cup E_{train}^{neg}$\;
Edge Probabilities, $P_{Edge} = \psi(E_{big})$\;
$\mathcal{D}_{Q} = \{(u,v,y) : (u,v) \in E_{big}, y= [{P_{edge}}_{[u,v]} > \zeta]\}$\;
\Return{$\mathcal{D}_{Q}$}\;
\end{func}


==> codaspyTex/function.tex <==
\section{Functions}\label{app:func}

\begin{func}[]
\renewcommand{\arraystretch}{1}
 \fontsize{8}{8}\selectfont
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Parameter}{Parameter}

\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
%\Comment{\textbf{Augmentation Module}: Get Cluster Centers for Node and Edge Augmentation, and generate the augmented graph, but with features not learned yet}

\Input{Graph $G = (V, \textbf{X}, \textbf{Y}, \textbf{A}, n, c);$\\}
\Parameter{Number of new nodes to augment, $n_{new}$;\\}
\Output{Augmented Graph $G_{aug} = (V_{aug}, \textbf{X}_{aug}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$ with no features learned yet;}

Cluster Center Nodes $[o_1, o_2, \ldots, o_{n_{new}}] \gets$ Spectral Clustering on $G$ as per the algorithm in~\cite{von2007tutorial}\; 
$V_{new} \gets \{v_1, v_2, \ldots v_{n_{new}}\},$ New nodes with zeroes set as feature\;
Form edge set $E_{new} \gets \{(o_1, v_1), (o_2,v_2), \ldots, (o_{n_{new}}, v_{n_{new}})\}$\;
$X_{new} \gets \{\mathbf{0}, \mathbf{0}, \mathbf{0}, \ldots, \mathbf{0}\}, $ $n_{new}$ zero feature vectors\;
$\mathbf{A}_{new} \gets $ form adjacency matrix as per \cref{eqn:anew} using $V, V_{new} \text{ \& } E_{new}$\;
$\mathbf{Y}_{new} \gets n_{new}$ randomly assigned labels from ${0,1,\ldots, c-1}$\;
Form augmented graph $G_{aug} = (V_{aug}, \textbf{X}_{aug}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$ using \cref{eqn:naugvaug,eqn:xaugaugyaug} \; 
\Return{$G_{aug}$}\;
\caption{getAugmentedGraph$(G)$}\label[func]{func:getAugGraph}
\end{func}

%\mir{WE HAVE TO TEST IT}
\begin{func}[]
\caption{runTriOptimizationBasedFeatureLearning$(G_{aug}, \mathcal{D}_Q)$}\label[func]{func:runtriopt}
\renewcommand{\arraystretch}{1}
 \fontsize{8}{8}\selectfont
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Parameter}{Parameter}
\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
\Input{Augmented Graph $G_{aug} = (V_{aug}, \textbf{X}_{aug}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$ with no features learned yet;\\Surrogate Query Edge Dataset $\mathcal{D}_{Q}$;\\}
\Parameter{number of epochs $\eta_{outer}, \eta_{class}, \eta_{surr}, \eta_{def}$;\\}
\Output{Learned Augmented Graph, $G_{aug}^{\tau} = (V_{aug}, \textbf{X}_{aug}^{\tau}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$;}
Initiate $\theta_g^{0},  \theta_{f_\tau}^{0}, \theta_{\tau}^{0}$\;
\For{$t=0$ to $\eta_{outer}-1$}{
\Comment{\textbf{Stage 1}: Learn Classification Model}
${{\hat{\theta}}_{f_\tau}^{0}}, {\hat{\theta}}_{\tau}^{0} \gets \theta_{f_\tau}^{t}, \theta_{\tau}^{t}$ \;
\For{$t_{c}=0$ to $\eta_{class}-1$}{
Calculate $\mathcal{L}_{class}(G_{aug}; {{\hat{\theta}}_{f_\tau}^{t_{c}},} {{\hat{\theta}}_{\tau}^{t_c})}$ using \cref{eqn:classloss}\;
$ {{\hat{\theta}}_{f_\tau}^{t_{c}+1}}, {{\hat{\theta}}_{\tau}^{t_{c}+1}} \gets $ Update using back-prop from $\mathcal{L}_{class}(G_{aug}; {{\hat{\theta}}_{f_\tau}^{t_{c}},} {{\hat{\theta}}_{\tau}^{t_c})}$\;}
\Comment{\textbf{Feature Learner Quasi-Update}}
${\theta_{f_\tau}^{t+1}}, {\theta_{\tau}^{t+\frac{1}{2}}}  \gets {{\hat{\theta}}_{f_\tau}^{\eta_{class}}},{{\hat{\theta}}_{\tau}^{\eta_{class}}} $\; 
\If{$t == 0$}{\Comment{\textbf{Stage 2}: Learn Surrogate Attacker Model}
${{\hat{\theta}}_{g}^{0}} \gets \theta_{g}^{t}  $ \;

\For{$t_{s}=0$ to $\eta_{surr}-1$}{
Calculate $\mathcal{L}_{attack}(\mathcal{D}_{Q},G_{aug};{{\hat{\theta}}_{g}^{t_s}},\theta_{f_\tau}^{t+1}, \theta_{\tau}^{t+\frac{1}{2}})$ using \cref{eqn:lossatk}\;
${{\hat{\theta}}_{g}^{t_s+1}}\gets $ Update using back-prop from $\mathcal{L}_{attack}(\mathcal{D}_{Q},G_{aug};{{\hat{\theta}}_{g}^{t_s}},\theta_{f_\tau}^{t+1}, \theta_{\tau}^{t+\frac{1}{2}})$\;}
\Comment{\textbf{Surrogate Attacker Update}}
$\theta_{g}^{t+1} \gets{{\hat{\theta}}_{g}^{\eta_{surr}}}$\;}
\Else{$\theta_{g}^{t+1} \gets \theta_{g}^{t}$}

\Comment{\textbf{Stage 3} Learn Augmented Features}
${{\hat{\theta}}_{\tau}^{0}}\gets \theta_{\tau}^{t+\frac{1}{2}} $\;
\For{$t_{d}=0$ to $\eta_{def}-1$}{
Calculate $\mathcal{L}_{defense}(\mathcal{D}_{Q}, G_{aug};\theta_{g}^{t+1},\theta_{f_\tau}^{t+1},{{\hat{\theta}}_{\tau}^{t_d}})$ using \cref{eqn:defloss}\;
${{\hat{\theta}}_{\tau}^{t_d+1}}\gets $ 
Update using back-prop from 
$\mathcal{L}_{defense}(\mathcal{D}_{Q}, G_{aug};\theta_{g}^{t+1},\theta_{f_\tau}^{t+1},{{\hat{\theta}}_{\tau}^{t_d}})$\;}
\Comment{\textbf{Feature Learner Final Update}}
$\theta_{\tau}^{t+1} \gets{{\hat{\theta}}_{\tau}^{\eta_{def}}}$\;

}
\Comment{$\theta_{\tau}^{\eta_{outer}}$ is the learned augmented node features}
$\mathbf{X}_{aug}^{\tau} \gets $ replace $\mathbf{X}_{new}$ from $\mathbf{X_{aug}}$ in \cref{eqn:xaugaugyaug} with $\theta_{\tau}^{\eta_{outer}}$\;
\Return{$G_{aug}^{\tau} = (V_{aug}, \textbf{X}_{aug}^{\tau}, \textbf{Y}_{aug}, \textbf{A}_{aug}, n_{aug}, c)$}

\end{func}

%%%%%%%%%%%%%%%%%%%%%%


==> tables/attackconfig.tex <==

\begin{table}[!htp]
\fixtableonecol{6}

 \caption{Attacker Knowledge Configurations for Link Stealing Attacks, as described in \cite{he2021stealing}}
    \label{tab:attack_config}
    \centering
    \begin{tabular}{c|c|c|c}
        Attack No. & $\mathcal{K} = (\mathcal{F}, \mathcal{A}, \mathcal{D'})$ & Attack No.  &  $\mathcal{K} = (\mathcal{F}, \mathcal{A}, \mathcal{D'})$\\\hline
       Attack:0  & $(\times, \times, \times)$ & Attack:4 & $(\times, \checkmark, \checkmark)$\\
       Attack:1  & $(\times, \times, \checkmark)$ & Attack:5 & $(\checkmark, \times, \checkmark)$\\
       Attack:2  & $(\checkmark, \times, \times)$ & Attack:6 & $(\checkmark, \checkmark, \times)$ \\
       Attack:3  & $(\times, \checkmark, \times)$  & Attack:7 & $(\checkmark, \checkmark, \checkmark)$\\\hline
    \end{tabular}
   
\end{table}
